Perturbative Quantization of Modified Maxwell Electrodynamics

Modified Maxwell electrodynamics, or ModMax for short, is the unique nonlinear extension of Maxwell's theory that preserves its notable symmetries: conformal invariance and electromagnetic duality. ModMax has been studied extensively at the classical level, however remains largely untouched in a quantum context due to its non-analytic nature. In this thesis, we perform the perturbative quantization of this theory. Using the background field method and dimensional regularization, we obtain novel corrections by calculating the one loop quantum effective action. These corrections vanish in a background with constant field strength, and are not of the form of the classical theory for a general background field. Motivated by the corrections obtained for ModMax, we applied the method developed to quantize ModMax to its two dimensional analogue theory. We similarly obtain the one loop quantum effective action for this theory in a general background by evaluating all one loop Feynman diagrams. In addition, we study the divergence of the separate infinite series of two vertex diagrams.

==> chapter/MM-BFM.tex <==
\chapter{ModMax in the Background Field Method}

As ModMax is not amenable to traditional quantization techniques, we quantize ModMax within the background field method.
\subsection{Background Field Splitting}

We can express ModMax in terms of $S = -\frac{1}{4} F_{\mu \nu} F^{\mu \nu}$ and $P = -\frac{1}{4} F_{\mu \nu} C^{\mu \nu}$ as
\begin{align*}
    \mathcal{L} = S \cosh \gamma  + \sinh \gamma \sqrt{S^2 + P^2} 
,\end{align*}
where we have
\begin{align*}
    F_{\mu \nu} = \partial_\mu A_\nu - \partial_\nu A_\mu  &&
    C^{\mu \nu} = \frac{1}{2} \epsilon^{\mu \nu \rho \sigma} F_{\rho\sigma}
.\end{align*}

We make a background field splitting of the form
\begin{align*}
    A_{\mu} \to C_{\mu} + a_{\mu}
,\end{align*}
where $C_{\mu}$ is classical and $a_\mu$ is a small quantum fluctuation. We then see that
\begin{align*}
    F_{\mu \nu} &\to \partial_{\mu} \left( C_{\nu} + a_{\nu} \right) - \partial_{\nu} \left( C_{\mu} + a_{\mu} \right)   \\
    &\equiv C_{\mu \nu} + f_{\mu \nu}
    \intertext{where we define these lowercase field strength tensors appropriately. We then see that}
    -4S = F_{\mu \nu} F^{\mu \nu} &\to \left( C_{\mu \nu} + f_{\mu \nu} \right) \left( C^{\mu \nu} + f^{\mu \nu} \right)  \\
    \intertext{and we assume the field strength tensor is constant with}
    \partial_\mu C_{\nu \rho} &= 0 \\
    F_{\mu \nu} F^{\mu \nu}&= C_{\mu \nu} C^{\mu \nu} + 2C_{\mu \nu} f^{\mu \nu} + f_{\mu \nu} f^{\mu \nu} \\
    \intertext{Focussing on the cross term we have}
    C_{\mu \nu} \left( \partial^\mu a^\nu \right) &= \partial^\mu \left( C_{\mu \nu} a^{\nu} \right) - \left( \partial^\mu C_{\mu \nu} \right) a^{\nu}   \\
    \intertext{where the second term vanishes due to the constraint and the first vanishes as it is a total derivative term we have}
    &= 0
    \intertext{and similarly}
    C_{\mu \nu} \left( \partial^\nu a^\mu \right) &= 0
    \intertext{and thus}
    C_{\mu \nu} f^{\mu \nu} &= 0
    \intertext{which reduces the expression to}
    S &= \underbrace{-\frac{1}{4}C_{\mu \nu} C^{\mu \nu}}_{S_C} -\frac{1}{2} C_{\mu \nu} f^{\mu \nu} - \frac{1}{4}f_{\mu \nu} f^{\mu \nu} \\
    S &= S_C - \frac{1}{4}f_{\mu \nu} f^{\mu \nu} \\
    \intertext{Note that the cross term does not vanish for $S^2$ and we instead have}
    S^2 &= S_C^2 - \frac{1}{2} S_C f_{\mu \nu} f^{\mu \nu} - S_C C_{\mu \nu} f^{\mu \nu} + \mathcal{O}\left( a^{3} \right) \\
    %S^2 &= S_C^2 - \frac{1}{2} S_C f_{\mu \nu} f^{\mu \nu} + \frac{1}{16} f_{\mu \nu} f^{\mu \nu} f_{\rho \tau} f^{\rho \tau} \\
    %S^2 &= S_C^2 - \frac{1}{2} S_C f_{\mu \nu} f^{\mu \nu} + \mathcal{O}\left( a^{4} \right) 
    \intertext{Similarly,}
    -4P = F_{\mu \nu} C^{\mu \nu} &= \left( C_{\mu \nu} + f_{\mu \nu} \right) \left( \frac{1}{2}\epsilon^{\mu \nu \rho \sigma} \left( C_{\rho\sigma} + f_{\rho\sigma} \right)  \right)  \\
    &= \frac{1}{2}\epsilon^{\mu \nu \rho \sigma}C_{\mu \nu} C_{\rho\sigma} + \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho\sigma} + \frac{1}{2} \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma} \\
    \intertext{The above argument is independent of the repeated indices and thus the cross term identically vanishes here, yielding}
    P&= \underbrace{-\frac{1}{8} \epsilon^{\mu \nu \rho \sigma}  C_{\mu \nu} C_{\rho\sigma}}_{P_C} - \frac{1}{4} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} - \frac{1}{8} \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma} \\
    P&= P_C - \frac{1}{8} \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma}
    \intertext{and thus}
    P^2 &= P_C^2 -\frac{1}{4} P_C \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma} - \frac{1}{2} P_C\epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} + \mathcal{O}\left( a^{3} \right)
    \intertext{Therefore considering the contents of the square root up to second order in $a$, we have}
    S^2 + P^2 &= S_C^2 + P_C^2 -\frac{1}{2}S_C f_{\mu \nu} f^{\mu \nu} - S_C C_{\mu \nu} f^{\mu \nu} - \frac{1}{4} P_C \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma} - \frac{1}{2} P_C \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \\
    %&= S_C^2 + P_C^2 - \frac{1}{2} S_C \left( f_{\mu \nu} + 2C_{\mu \nu} \right) f^{\mu \nu} - \frac{1}{4}P_C \epsilon^{\mu \nu \rho \sigma} \left( f_{\mu \nu} + 2 C_{\mu \nu} \right) f_{\rho \sigma}   \\
    %&= S_C^2 + P_C^2 - \left( \frac{1}{2} S_C f^{\mu \nu} + \frac{1}{4}P_C \epsilon^{\mu \nu \rho \sigma} f_{\rho \sigma}\right)  \left( f_{\mu \nu} + 2 C_{\mu \nu} \right)    \\
    \intertext{where we define}
    S^2 + P^2 &= S_C^2 + P_C^2 + Q
.\end{align*}


Therefore, taking a Taylor series expansion of the square root we have up to quadratic terms in $a$,
\begin{align*}
    %\sqrt{S_C^2 + P_C^2 + Q}  \to \sqrt{S_C^2 + P_C^2 } + \frac{Q}{2 \sqrt{S_C^2 + P_C^2} } - \frac{Q^2}{8 \left( S_C^2 + P_C^2 \right)^{\frac{3}{2}}}
    \sqrt{S_C^2 + P_C^2 + Q}  \to \sqrt{S_C^2 + P_C^2 } + \frac{Q}{2 \sqrt{S_C^2 + P_C^2} } - \frac{Q^2}{8 \left( S_C^2 + P_C^2 \right)^{\frac{3}{2}}}
.\end{align*}

Note that for $Q$ we have some topological terms that cancel with 
\begin{align*}
    Q &= -\frac{1}{2}S_C f_{\mu \nu} f^{\mu \nu} - S_C C_{\mu \nu} f^{\mu \nu} - \frac{1}{4} P_C \epsilon^{\mu \nu \rho \sigma} f_{\mu \nu} f_{\rho\sigma} - \frac{1}{2} P_C \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \\
    Q &= -\frac{1}{2}S_C f_{\mu \nu} f^{\mu \nu}
.\end{align*}

Expanding $Q^2$ up to quadratic terms in $a$ we have
\begin{align*}
    Q^2 &= \left( S_C C_{\mu \nu} f^{\mu \nu} \right)^2 + \left( \frac{1}{2} P_C \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \right)^2  + S_C P_C C_{\gamma \tau} f^{\gamma \tau} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma}
.\end{align*}
Therefore, overall we have
\begin{align*}
    \mathcal{L} &\to \mathcal{L}_C - \frac{1}{4} f_{\mu \nu} f^{\mu \nu} - \frac{\frac{1}{2}S_C f_{\mu \nu} f^{\mu \nu} }{2 \sqrt{S_C^2 + P_C^2} }\\
                &\phantom{=}- \frac{\left( S_C C_{\mu \nu} f^{\mu \nu} \right)^2 + \left( \frac{1}{2} P_C \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \right)^2  + S_C P_C C_{\gamma \tau} f^{\gamma \tau} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma}}{8 \left( S_C^2 + P_C^2 \right)^{\frac{3}{2}}} \\
    &= \mathcal{L}_C - \frac{1}{4} f_{\mu \nu} f^{\mu \nu} - \frac{S_C f_{\mu \nu} f^{\mu \nu} }{4 \sqrt{S_C^2 + P_C^2} } \\
        &\phantom{=}- \frac{S_C^2 C_{\mu \nu} f^{\mu \nu} C_{\rho \tau} f^{\rho \tau}+ \left( \frac{1}{2} P_C \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \right)^2  + S_C P_C C_{\gamma \tau} f^{\gamma \tau} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma}}{8 \left( S_C^2 + P_C^2 \right)^{\frac{3}{2}}}
.\end{align*}

%\begin{align*}
%    \left( \partial_\nu A_\mu \right) \left( \partial^{\mu} A^{\nu} \right) &= \partial_\nu \left( A_\mu \partial^{\mu} A^{\nu} \right) - A_{\mu} \left( \partial_\nu \partial^{\mu} A^{\nu} \right)  \\
%    A_{\mu} \left( \partial^{\mu} \partial_\nu A^{\nu}\right)  &= \partial^{\mu} \left( A_{\mu} \partial_\nu A^{\nu} \right) - \left( \partial^\mu A_{\mu} \right)^2  \\
%    \implies \left( \partial_\nu A_\mu \right) \left( \partial^{\mu} A^{\nu} \right) &= \partial_\nu \left( A_\mu \partial^{\mu} A^{\nu} - A^{\nu} \partial^{\mu} A_{\mu} \right) + \left( \partial^{\mu} A_{\mu} \right)^2
%.\end{align*}
%
%\begin{align*}
%    \left( \partial_\nu A_\mu \right) \left( \partial^{\mu} a^{\nu} \right) &= \partial_\nu \left( A_\mu \partial^{\mu} a^{\nu} \right) - A_{\mu} \left( \partial_\nu \partial^{\mu} a^{\nu} \right)  \\
%    A_{\mu} \left( \partial^{\mu} \partial_\nu a^{\nu}\right)  &= \partial^{\mu} \left( A_{\mu} \partial_\nu a^{\nu} \right) - \left( \partial^\mu A_{\mu} \right) \left( \partial^{\nu} a_{\nu} \right)   \\
%    \implies \left( \partial_\nu A_\mu \right) \left( \partial^{\mu} a^{\nu} \right) &= \partial_\nu \left( A_\mu \partial^{\mu} a^{\nu} - A^{\nu} \partial^{\mu} a_{\mu} \right) + \left( \partial^{\mu} A_{\mu} \right) \left( \partial^{\nu} a_\nu \right) 
%.\end{align*}

%\begin{align*}
%    \sqrt{S_C^2 + P_C^2 + L}  \to \sqrt{S_C^2 + P_C^2 } + \underbrace{\frac{1}{2} R_C^{-1} L}_{\text{vanish}} + \frac{1}{4} R_C^{-3} L^2  
%.\end{align*}
\subsection{Finding $P^{\mu \nu}$}

Next, we want this written as
\begin{align*}
    \mathcal{L} = \mathcal{L}_{C} + a_{\mu} P^{\mu \nu} a_{\nu}
,\end{align*}
such that we can invert $P^{\mu \nu}$. The first term separates as
\begin{align*}
     \left( \partial_\mu a_\nu \right) f^{\mu \nu} &= -a_{\nu} \partial_\mu f^{\mu \nu} \\
     \implies -\frac{1}{4}f_{\mu \nu} f^{\mu \nu} &= \frac{1}{2} a_\nu \partial_\mu\partial^{\mu} a^{\nu} - \frac{1}{2} a_{\mu} \partial_{\nu}\partial^{\mu} a^{\nu} \\
     &= \frac{1}{2} a_{\nu} \partial_\mu \partial^{\mu} g^{\rho \nu} a_{\rho} - \frac{1}{2} a_{\mu} \partial_\nu \partial^{\mu} g^{\nu \rho} a_{\rho} \\
     \intertext{Relabelling}
    &= \frac{1}{2} a_{\mu} \partial_\rho \partial^{\rho} g^{\mu\nu} a_{\nu} - \frac{1}{2} a_{\mu} \partial_\rho \partial^{\mu} g^{\rho \nu} a_{\nu} \\
    &= \frac{1}{2}a_{\mu} \left( \partial_\rho \partial^{\rho} g^{\mu\nu} - \partial_\rho \partial^{\mu} g^{\rho \nu} \right) a_\nu  \\
    &= \frac{1}{2}a_{\mu} \left( \partial_\rho \partial^{\rho} g^{\mu\nu} - \partial^\nu \partial^{\mu} \right) a_\nu
.\end{align*}

We analogously have
\begin{align*}
    C_{\mu \nu} \partial^{\mu} a^{\nu} C_{\rho \tau} f^{\rho \tau} &= - a^{\nu} \partial^{\mu} \left( C_{\mu \nu} C_{\rho \tau} f^{\rho \tau} \right)  \\
    &= - a^{\nu} C_{\mu \nu} C_{\rho\tau} \partial^{\mu} f^{\rho \tau} \\
    &= -2a^{\nu} C_{\mu \nu} C_{\rho\tau} \partial^{\mu} \partial^{\rho} a^{\tau}   \\
    \intertext{therefore}
    C_{\mu \nu} f^{\mu \nu} C_{\rho \tau} f^{\rho \tau} &= -2\left( a^{\nu} C_{\mu \nu} C_{\rho\tau} \partial^{\mu} - a^{\mu} C_{\mu \nu} C_{\rho \tau} \partial^{\nu} \right)  \partial^{\rho} a^{\tau} \\
    &= -2\left( a^{\nu} C_{\mu \nu} C_{\rho\tau} \partial^{\mu} - a^{\nu} C_{\nu \mu} C_{\rho\tau} \partial^{\mu} \right)  \partial^{\rho} a^{\tau} \\
    &= -4a^{\nu} C_{\mu \nu} C_{\rho \tau} \partial^{\mu} \partial^{\rho} a^{\tau} \\
    &= -4a_{\mu} g^{\mu \tau} C_{\gamma \tau} C_{\rho \sigma} g^{\sigma \nu} \partial^{\gamma} \partial^{\rho} a_{\nu}  \\
    &= -4 a_{\mu} \tensor{C}{_{\gamma}^{\mu}} \tensor{C}{_{\rho} ^{\nu}} \partial^{\gamma} \partial^{\rho} a_{\nu} \\
    \intertext{and similarly,}
    C_{\gamma \tau} f^{\gamma \tau} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} &= -4a^{\tau} C_{\gamma \tau} \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu}  \partial^{\gamma} \partial_{\rho} a_{\sigma} \\
    &= -4 a_{\mu} C^{\gamma \mu} \epsilon^{\tau \sigma \rho \nu} C_{\tau \sigma} \partial_{\gamma} \partial_{\rho} a_{\nu} \\
    \intertext{and}
    \epsilon^{\mu \nu \rho \sigma} C_{\mu \nu} f_{\rho \sigma} \epsilon^{\gamma \tau \alpha \beta} C_{\gamma \tau} f_{\alpha \beta}  &= -4 a_{\sigma}\epsilon^{\mu \nu \rho \sigma}  C_{\mu \nu} \epsilon^{\gamma \tau \alpha \beta} C_{\gamma \tau} \partial_{\rho} \partial_{\alpha} a_{\beta} \\
    &= -4a_{\mu} \epsilon^{\sigma \beta \rho \mu} C_{\sigma \beta} \epsilon^{\gamma \tau \alpha \nu} C_{\gamma \tau} \partial_{\rho} \partial_{\alpha} a_\nu
.\end{align*}

\subsection{Result}
We then have
\begin{align*}
    P^{\mu \nu} &= \frac{1}{2}\left( 1 + \frac{S_C}{\sqrt{S_C^2 + P_C^2} } \right)  \left( \partial_\rho \partial^{\rho} g^{\mu\nu} - \partial^\nu \partial^{\mu} \right) \\
                &\phantom{=} + \left( \frac{1}{2\left( S_C^2 + P_C^2 \right)^{\frac{3}{2}} } \right) \left( S_C^2 \tensor{C}{_{\gamma}^{\mu}} \tensor{C}{_{\rho} ^{\nu}} \partial^{\gamma} \partial^{\rho} + S_CP_CC^{\gamma \mu} \epsilon^{\tau \sigma \rho \nu} C_{\tau \sigma} \partial_{\gamma} \partial_{\rho} + \frac{P_C^2}{4}\epsilon^{\sigma \beta \rho \mu} C_{\sigma \beta} \epsilon^{\gamma \tau \alpha \nu} C_{\gamma \tau} \partial_{\rho} \partial_{\alpha} \right) \\
                \intertext{or alternatively writing the Hodge dual of the classical field strength tensor as $\tilde{C}^{\mu \nu} = \frac{1}{2}\epsilon^{\mu \nu \rho \tau} C_{\rho \tau}$, we can compress this to}
    P^{\mu \nu} &= \frac{1}{2}\left( 1 + \frac{S_C}{\sqrt{S_C^2 + P_C^2} } \right)  \left( \partial_\rho \partial^{\rho} g^{\mu\nu} - \partial^\nu \partial^{\mu} \right) \\
                %&\phantom{=} + \left( \frac{1}{2\left( S_C^2 + P_C^2 \right)^{\frac{3}{2}} } \right) \left( S_C^2 C^{\gamma \mu} C^{\rho \nu} \partial_{\gamma} \partial_{\rho} + S_CP_CC^{\gamma \mu} \tilde{C}^{\rho \nu} \partial_{\gamma} \partial_{\rho} + \frac{P_C^2}{4}\tilde{C}^{\gamma \mu}  \tilde{C}^{\rho \nu} \partial_{\gamma} \partial_{\rho} \right)
    &\phantom{=} + \left( \frac{1}{2\left( S_C^2 + P_C^2 \right)^{\frac{3}{2}} } \right) \left( S_C^2 C^{\gamma \mu} C^{\rho \nu}  + 2S_CP_CC^{\gamma \mu} \tilde{C}^{\rho \nu}  + P_C^2\tilde{C}^{\gamma \mu}  \tilde{C}^{\rho \nu}  \right)\partial_{\gamma} \partial_{\rho}
    % below is attempt to factorize
%    P^{\mu \nu} &= \frac{1}{2}\left( 1 + \frac{S_C}{\sqrt{S_C^2 + P_C^2} } \right)  \left( \partial_\rho \partial^{\rho} g^{\mu\nu} - \partial^\nu \partial^{\mu} \right) \\
%    &\phantom{=} + \left( \frac{1}{2\left( S_C^2 + P_C^2 \right)^{\frac{3}{2}} } \right) \left( S_C C^{\gamma \mu} + P_C \tilde{C}^{\rho \nu}  \right) \left( S_C C^{\rho \nu} + P_C \tilde{C}^{\gamma \mu} \right) \partial_{\gamma} \partial_{\rho}
.\end{align*}


\begin{claim}
    Topological terms vanish.   
\end{claim}

\begin{proof}
    Identically, we have
    \begin{align*}
        -\epsilon^{\mu \nu \rho \sigma}f_{\mu \nu} f_{\rho \sigma} &= \epsilon^{\mu \nu \rho \sigma}\left( a_\nu\partial_\mu  \partial_\rho a_\sigma - a_\nu\partial_\mu  \partial_\sigma a_\rho - a_\mu\partial_\nu  \partial_\rho a_\sigma + a_\mu\partial_\nu  \partial_\sigma a_\rho  \right) \\
         &= \epsilon^{\mu \nu \rho \sigma}\left( 2a_\nu\partial_\mu  \partial_\rho a_\sigma   + 2a_\mu\partial_\nu  \partial_\sigma a_\rho  \right) \\
        &= \epsilon^{\mu \nu \rho \sigma}\left( 4a_\mu\partial_\nu  \partial_\sigma a_\rho  \right)
        \intertext{Relabelling}
        &= a_{\mu} \left( 4 \epsilon^{\mu \rho \nu \sigma}  \partial_\rho \partial_\sigma \right) a_\nu
    .\end{align*}

\end{proof}

\section{To Be Distributed}

Using the background field method and gauge fixing technique outlined above, I have successfully obtained the Feynman rules for ModMax and applied them to evaluate all Feynman diagrams containing one loop. This means ModMax has successfully been quantized up to one loop.

To achieve this, the propagator $D^{\nu \rho}$ for the ModMax quantum photon field was found to satisfy
\begin{align}
    -\cosh \gamma k^2 g_{\mu \nu} D^{\nu \rho} &=  i \delta_{\mu}^{\rho} \\
    \intertext{which is very similar to that occurring in QED. As such it admits a similar solution given by}
    \implies D^{\nu \rho}  &= \frac{1}{\cosh \gamma} \frac{-i g^{\nu \rho}}{k^2 + i \epsilon}
.\end{align}

The vertex factor however, due to the nonlinearity caused by the square root in ModMax departs significantly from the form observed in QED.

I will draw quantum photon fields as wavy lines and the background photon field as an unlabelled solid line. The vertex factor was found to be
\begin{align}
    \vcenter{\hbox{
                            \begin{tikzpicture}
                            \begin{feynman}
    \diagram [small,horizontal=a to d] {
        a -- [photon,momentum=$p\text{, }\nu$] e [dot, label=0:$ $],  
        b -- [photon, momentum'=$p\text{, }\mu$] e, 
        e -- c [crossed dot];
        e -- d [crossed dot];
    }; \end{feynman} \end{tikzpicture} }} &= -2\sinh \left( \gamma \right) \left( S_C p^2 g^{\mu \nu} + 4 B^{\alpha \nu \beta \mu} p_{\alpha} p_{\beta}   \right) 
,\end{align}
where $S_C$ and $B^{\alpha \nu \beta \mu}$ capture nonlinearity associated with the background field. The exact form of these quantities are not important as the quantum photon field is the object of interest.

This vertex allows us to calculate the series of diagrams (shown below) that sum to yield the quantum corrections predicted by ModMax.
\begin{align}
        \feynmandiagram [horizontal=a to b, spring layout, baseline=(a.base)] {
        a -- [photon, half left, looseness=1.5] b [dot, label=0:$ $], 
        a -- [photon, half right, looseness=1.5, ] b , % rmomentum'=$k\text{, }\mu$
        b -- c [crossed dot];
        b -- d[crossed dot];
    }; 
    +
        \feynmandiagram [horizontal=a to b, spring layout, baseline=(a.base)] {
            f [crossed dot] -- a [dot];
        g [crossed dot] -- a;
        a -- [photon, half left, looseness=1.5] b [dot, label=0:$ $], 
        a -- [photon, half right, looseness=1.5, ] b , % rmomentum'=$k\text{, }\mu$
        b -- c [crossed dot];
        b -- d [crossed dot];
    }; + 
\feynmandiagram [horizontal=a to d, spring layout, baseline=(a.base)] {
    i1 [crossed dot] -- a [dot],
    i2 [crossed dot] -- a 
  -- [photon, quarter left] c [dot]
  -- [photon, quarter left] d [dot]
  -- [photon, quarter left] a,
  c -- f1 [crossed dot],
  c -- f3 [crossed dot],
  d -- f2 [crossed dot],
  d -- f4 [crossed dot]
}; + \cdots
.\end{align}

The first two diagrams were evaluated by hand using the propagator as well as vertex factor derived and were shown to be exactly zero. For the full calculation, see Appendix A. This argument was generalized to work for all such diagrams containing one loop. This infinite series of diagrams was shown to contribute exactly zero additional quantum corrections to the classical equations of ModMax. 

In addition, the first two diagrams (suppressing external classical field lines) containing two loops that contribute most significantly (shown below) were also evaluated by hand using the Feynman rules derived.
\begin{align*}
    \vcenter{\hbox{
                            \begin{tikzpicture}
                            \begin{feynman}
    \diagram [horizontal=a to c] {
        a -- [photon, half left, looseness=1.5] b [dot, label=0:$ $], 
        a -- [photon, half right, looseness=1.5, ] b,
        b -- [photon, half left, looseness=1.5, ] c,
        b -- [photon, half right, looseness=1.5] c;
    }; \end{feynman} \end{tikzpicture} }}
\vcenter{\hbox{
    \begin{tikzpicture}
    \begin{feynman}
    \diagram [horizontal=a to c] {
        a [dot] -- [photon, half left, looseness=1.5] b [dot, label=0:$ $], 
        a -- [photon, half right, looseness=1.5] b, %, momentum'=$k\text{, }\rho$
        b -- [photon, half left, looseness=1.5] c, 
        b -- [photon, half right, looseness=1.5, ] c ; % rmomentum'=$k\text{, }\mu$
    }; \end{feynman} \end{tikzpicture}
}}
,\end{align*}
It was shown that these diagrams also both vanish identically. Lastly, a third two loop diagram was also evaluated and yielded an expression
\begin{align}
            \vcenter{\hbox{
        \begin{tikzpicture}
\begin{feynman}
    \diagram [horizontal=b to c] {
        c [dot] -- [photon, half right, momentum'=$p$] b [dot, label=0:$ $], 
        b -- [photon,momentum'=$q$] c, 
        c -- [photon, half left, rmomentum=$p-q$] b, 
}; \end{feynman} \end{tikzpicture} }}
    &=  \int \frac{\dd{^{d}q}}{\left( 2\pi \right)^{d}} \frac{q_{\rho_1} q_{\rho_2} q_{\alpha_1} q_{\alpha_2}}{q^2} \frac{i\Gamma\left( 1 - \frac{d}{2} \right)}{\left( 4\pi \right)^{\frac{d}{2}} \left( d-1 \right)  }\left[ q_{\mu_1} q_{\mu_2} q^{d-4} \left( 1 - \frac{d}{2} \right) - \frac{dg_{\mu_1 \mu_2}}{8}  q^{d-2}  \right]
,\end{align}
where $d$ is the dimension of spacetime and $\Gamma \left( n \right) = \left( n + 1 \right)!$, is the extension of the factorial to non-integers. This expression diverges when we take $d = 4$, however if we take the limit as $d$ approaches $4$, then we obtain finite values for all $d = 4 + \epsilon$ with $\epsilon > 0$. The removal of the divergence in this fashion is the subject of the renormalization of this theory, which is one possible natural continuation of this project.

\section{Next Steps}

Proceeding further in this manner of increasing loop order is impractical but we expect that a generalization can be made to suggest that all diagrams should vanish for any number of loops. With this simpler case evaluated, the natural next step is to move to the case in which we allow the classical background field to vary both in space and time. From preliminary calculations, this will lead to nonzero contributions from diagrams containing any number of loops. The introduction of non-constant background fields in this manner is the current next step in the project and is currently underway.

The nonzero contribution in this case is of particular interest as it will be logarithmically divergent, and thus has the potential to lead to a novel class of conformally invariant classical models generated quantum mechanically through ModMax.

Additionally, there is an analogue of ModMax in $d = 2$ dimensions that studies a system of $N$ boson fields instead of a photon field. The techniques I have applied and the procedure I have developed so far for ModMax generalize to this related theory. The study of this analogue theory and it's quantum properties is also underway.


==> chapter/defs_thesis.tex <==
% Copyright (C) 2004 Paul Cochrane
% 
% This program is free software; you can redistribute it and/or
% modify it under the terms of the GNU General Public License
% as published by the Free Software Foundation; either version 2
% of the License, or (at your option) any later version.
%   
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
%    
% You should have received a copy of the GNU General Public License
% along with this program; if not, write to the Free Software
% Foundation, Inc., 59 Temple Place - Suite 330, Boston, MA  02111-1307, USA.

\newcommand {\tbf}[1] {\textbf{#1}}
\newcommand {\tit}[1] {\textit{#1}}
\newcommand {\tmd}[1] {\textmd{#1}}
\newcommand {\trm}[1] {\textrm{#1}}
\newcommand {\tsc}[1] {\textsc{#1}}
\newcommand {\tsf}[1] {\textsf{#1}}
\newcommand {\tsl}[1] {\textsl{#1}}
\newcommand {\ttt}[1] {\texttt{#1}}
\newcommand {\tup}[1] {\textup{#1}}

\newcommand {\mbf}[1] {\mathbf{#1}}
\newcommand {\mmd}[1] {\mathmd{#1}}
\newcommand {\mrm}[1] {\mathrm{#1}}
\newcommand {\msc}[1] {\mathsc{#1}}
\newcommand {\msf}[1] {\mathsf{#1}}
\newcommand {\msl}[1] {\mathsl{#1}}
\newcommand {\mtt}[1] {\mathtt{#1}}
\newcommand {\mup}[1] {\mathup{#1}}

\newcommand {\figwidth} {100mm}
%\newcommand {\Ref}[1] {Reference~\cite{#1}}
\newcommand {\Sec}[1] {Section~\ref{#1}}
\newcommand {\App}[1] {Appendix~\ref{#1}}
\newcommand {\Chap}[1] {Chapter~\ref{#1}}
\newcommand {\etal} {\emph{~et~al.}}
\newcommand {\bul} {$\bullet$ }   % bullet
%\newcommand {\fig}[1] {Figure~\ref{#1}}   % references Figure x
%\newcommand {\imp} {$\Rightarrow$}   % implication symbol (default)
%\newcommand {\impt} {$\Rightarrow$}   % implication symbol (text mode)
%\newcommand {\impm} {\Rightarrow}   % implication symbol (math mode)
%\newcommand {\vect}[1] {\mathbf{#1}} 
%\newcommand {\hvect}[1] {\hat{\mathbf{#1}}}
%\newcommand {\del} {\partial}
%\newcommand {\eqn}[1] {Equation~(\ref{#1})} 
%\newcommand {\tab}[1] {Table~\ref{#1}} % references Table x
%\newcommand {\half} {\frac{1}{2}} 
%\newcommand {\ten}[1] {\times10^{#1}}
%\newcommand {\bra}[2] {\mbox{}_{#2}\langle #1 |}
%\newcommand {\ket}[2] {| #1 \rangle_{#2}}
%\newcommand {\Bra}[2] {\mbox{}_{#2}\left.\left\langle #1 \right.\right|}
%\newcommand {\Ket}[2] {\left.\left| #1 \right.\right\rangle_{#2}}
%\newcommand {\im} {\mathrm{Im}}
%\newcommand {\re} {\mathrm{Re}}
%\newcommand {\braket}[4] {\mbox{}_{#3}\langle #1 | #2 \rangle_{#4}} 
%\newcommand {\dotprod}[4] {\mbox{}_{#3}\langle #1 | #2 \rangle_{#4}} 
%\newcommand {\trace}[1] {\text{tr}\left(#1\right)}

% spell things correctly
\newenvironment{centre}{\begin{center}}{\end{center}}
\newenvironment{itemise}{\begin{itemize}}{\end{itemize}}

\usepackage{play}
\usepackage[grey,times]{quotchap}
\usepackage{makeidx}

%%%%% set up the bibliography style
\bibliographystyle{uqthesis}  % uqthesis bibliography style file, made
			      % with makebst

%%%%% optional packages
\usepackage[square,comma,numbers,sort&compress]{natbib}
		% this is the natural sciences bibliography citation
		% style package.  The options here give citations in
		% the text as numbers in square brackets, separated by
		% commas, citations sorted and consecutive citations
		% compressed 
		% output example: [1,4,12-15]

\usepackage[nottoc]{tocbibind}  
				% allows the table of contents, bibliography
				% and index to be added to the table of
				% contents if desired, the option used
				% here specifies that the table of
				% contents is not to be added.
				% tocbibind needs to be after natbib
				% otherwise bits of it get trampled.

\usepackage{amsmath,amsfonts,amssymb} % this is handy for mathematicians and physicists
			      % see http://www.ams.org/tex/amslatex.html

% \usepackage{showkeys} % this shows what labels you are using for cross
		      % references

\usepackage{graphicx} % standard graphics package for inclusion of
		      % images and eps files into LaTeX document

\usepackage{epsfig} % older graphics package for inclusion of eps
		    % files into LaTeX document

% this code hacked from that of R Chandrasekhar from UWA
\newif\ifpdf
\ifx\pdfoutput\undefined
	\pdffalse    % we are not running pdfLaTeX
\else
	\pdfoutput=1 % we are running pdfLaTeX
	\pdftrue
\fi

\ifpdf
	\DeclareGraphicsExtensions{.pdf}  % this command defined in graphicx
	\pdfcompresslevel=9  % 0: no compression, 9: highest compression
			     % or, set compress_level 9 in file pdftex.cfg
\else
	\DeclareGraphicsExtensions{.ps}
\fi

% put in an index?
% \makeindex


==> front/publications.tex <==
\chapter{List of Publications}

\begin{itemize}
\item[\bul] insert author list \emph{insert paper title}.  (submitted to
	insert journal name)
\item[\bul] insert author list \emph{insert paper title}.  
        insert journal name \textbf{insert volume number}, 
        insert article or page number (insert year)
\end{itemize}

